A Complete Criterion for Value of Information in Soluble Influence Diagrams

Influence diagrams have recently been used to analyse the safety and fairness properties of AI systems. A key building block for this analysis is a graphical criterion for value of information (VoI). This paper establishes the first complete graphical criterion for VoI in influence diagrams with multiple decisions. Along the way, we establish two important techniques for proving properties of multi-decision influence diagrams: ID homomorphisms are structure-preserving transformations of influence diagrams, while a Tree of Systems is collection of paths that captures how information and control can flow in an influence diagram.

==> definitions/voc.tex <==









\chris{Surely Tom didn't invent VoC}
\ryan{VoC goes back to at least \citet{shachter1986evaluating}.
It's just this specific phrasing that's from Tom.}
\begin{restatable}[\citet{Everitt2021agent}]{definition}{defvoc}
Let $(\calG, P)$ be a CIM with a chance node $X \in \sX$,
and let $\Pi$ be the set of policies.
Then the \emph{value of control} of $X$ is:
    \[
    \max_{\spi \in \Pi}\max_{g^X} \EE_\spi[\totutilvar|do(X=g^X(\pa_x))]
    -
    \max_{\spi \in \Pi} \EE_\spi[\totutilvar]
\]
where $g^X$ is a soft intervention at $X$, i.e.\ a new CPD for $X$ that respects the graph.
\end{restatable}

==> sections/1.4-voc-completeness.tex <==
\section{The Taskify Theorem \& Value of Control} \label{sec:voc-completeness-main} %
Value of control describes how much utility an agent could gain
by controlling one extra variable \citep{Matheson1990}.~\looseness=-1

\input{definitions/voc}

Our second main result is a sound and complete criterion for VoC.

\input{theorems/voc}

To prove the soundness direction (\cref{app:soundness}), 
we note that whatever CPD $g^X$ is 
selected, there always exists a policy $\pi$, optimal in $\calM_{g^X}$, that
factors over the minimal d-reduction. Under that $\pi$, changing the CPD of 
$X$ cannot change performance, so in particular, replacing $g^X$ with the non-intervened CPD $p^X$ cannot change performance. Thus any performance that 
can be obtained with an intervention $g^X$ can also be attained without.



To prove the completeness direction, it will suffice to prove that the path $p$ 
carries an effect from $X$ to some $U \in \sU$, so that $U$ 
takes a higher value if an intervention $g^X$ is performed.
In the single-decision case, all nodes on $p$ are chance nodes, so we can simply choose CPDs that copy the value along $p$. 
In the multi-decision case, 
however, 
there may be some decisions on $p$, whose CPDs are chosen by the agent. Thus the problem is to require these decisions to copy their predecessor.
\ryan{Maybe change Taskify out of mathmode?}
To do this, we propose a general procedure called \emph{Taskify}
that generalizes the construction used for completeness of VoI, 
to force \emph{any} decision in the CID to perform an arbitrary task. 
Specifically, for any CID with SR, and any deterministic decision rule $\pi^{D'}$ for $D'$, Taskify constructs a model that requires $D'$ to follow $\pi^{D'}$,
in order to perform optimally. In this way, we can construct a model by ``assigning tasks" to decisions.~\looseness=-1

Formally, Taskify takes a model, and a set of tasks, and generates an extended model on an extended graph (using \cref{le:21may19.2-CID-hom-from-node-copying-and-deleting}). We call such an extension a \textit{homomorphic extension}:~\looseness=-1



\input{theorems/Taskify}


Intuitively, \cref{le:21jan31.3-multi-Taskify-lemma} says that CID graphs are compatible with a wide range of optimal responses to requisite observations.
Condition (b) implies that the added utility nodes are unaffected by interventions inside the support of the intervened variable, which is important for using Taskify to establish properties like VoC.

Using Taskify, we can prove the completeness of graphical criteria in the following steps: (1) Construct a model on the chance nodes and utility nodes; (2) Assign tasks to the decision nodes using Taskify to obtain an extended model,
and show that the property (e.g. VoC) is satisfied;
(3) prove that the property (e.g. VoC) is preserved along the CID homomorphism, so also present in the original graph.
We do this for VoC, and we suggest Taskify may be analogously used for other properties: 








\begin{proof}[Proof of \cref{thm:voc} (Completeness direction)]
\newcommand{\Minitial}{\calM^\mathrm{init}}
Let $\Minitial$ be a model on $\sG$ where 
$P(X=1)=\varepsilon$, $P(X=0)=1-\varepsilon$, $\dom(X)=\{0,1\}$, each other 
chance node 
on $X \pathto U$
copies 
the value of its predecessor, 
and all other nodes have trivial domains.
Then obtain $(\GTaskify, \MTaskify)$ with $h\colon \GTaskify\to \sG$ by 
assigning $\piTask^{D^i}=\delta(d,x)$ the identity function for each $D^i$ on the path (\cref{le:21jan31.3-multi-Taskify-lemma}).
We show there is positive VoC on $X$ in $\MTaskify$: Take any optimal $\pi$ on $\MTaskify$. Since $X$ has full support in $\Minitial$, $X$ also has
full support in the homomorphic extension $\MTaskify$. So,
by \cref{le:21jan31.3-multi-Taskify-lemma} \ref{le:21jan31.3a-taskify-optimal-iff-performs-task}, 
each decision has $\pi^{D^i}(d|\pa)=\piTask^{D^i}(d|\pa)=\delta(d,x)$ with probability 1
under any intervention $g^X$ \chris{Change to be about equals pitask with prob 1.}, 
so that $U=X$, hence $\EE_{\pi}^{\MTaskify}(U | do(X=1)) = 1$, while $\EE_{\pi}^{\MTaskify}(U) = \varepsilon$. 
By \cref{le:21jan31.3-multi-Taskify-lemma} \ref{le:21jan31.3c-taskify-added-utility-nodes-unaffected}, the added utility nodes have constant value (also using full support of $X$). Hence, the VoC on $X$ equals $1-\varepsilon>0$ in $\MTaskify$. Finally, since the CID homomorphism $h$ preserves VoC (\cref{th:CID-homomorphism-preserves-VoC}), the VoC on $h(X)$ in the model $h(\MTaskify)$ on $\sG$ is also positive.~\looseness=-1 
\end{proof}

==> sections/2.1-soundness-proofs.tex <==








\clearpage
\section{Soundness result} \label{app:soundness}
\pagestyle{plain}
\pagenumbering{arabic}
\renewcommand*{\thepage}{A-\arabic{page}}


In this section, we use a lemma from \citet{nilsson2000evaluating}, 
to prove the soundness of a criterion for value of information.

We will use some language for talking about policies across different graphs, %
consistent with the past usage of \citet{nilsson2000evaluating}.
First, if $\calM(\calG)$ is a CIM on a CID $\calG$, and $\calG'$ is like $\calG$ but missing some information links, then $\calM$ immediately also defines a CIM $\calM(\calG')$ on $\calG'$.
If $\pi'$ is a rule for $D$ in $\calM(\calG')$, then $\pi'$ can be typecast into a policy for $\calM(\calG)$ via $\pi'(\tilde\pa^D, \pa^D\setminus\tilde\pa^D, \eps^D) := \pi'(\tilde\pa^D, \eps^D)$, where $\tilde\Pa^D$ are the parents of $D$ in $\calG'$.
We will therefore allow ourselves to talk about policies for $\calM(\calG')$ as policies also for $\calM(\calG)$.

The result from \citet{nilsson2000evaluating} is as follows.

\input{theorems/nonrequisite-removal}

Intuitively, the proof (\citep[Theorem 3]{nilsson2000evaluating}) shows that performance is not decreased whenever a nonrequisite
link is removed, and induction is performed over successive $d$-reductions.

\ryan{Change this to refer to VoI}
\chris{Should we cite, to clarify we didn't come up with this?}
\begin{corollary}[VoI graphical criterion soundness] \label{le:materiality-soundness}
Let $\calG$ be a CID \withSR containing a decision $D \in \sD$ and chance node $X \in \Pa(D)$.
If the minimal d-reduction $\calG^*$ does not contain $X \to D$
then 
in every CIM $\calM$ compatible with $\calG$,
$X$ has positive VoI for $D$.
\end{corollary}

The result follows immediately from \cref{le:dred-performance}.





==> sections/2.9-taskify.tex <==


\section{The Taskify Theorem}\label{sec:Taskify-construction}
We will now generalize the model for materiality into the $\sTaskify$ construction, which will essentially: (1) construct a transformed CID that contains the original CID, but has a normal form tree (by \autoref{le:20nov29.1-Existence-of-adequate-CID-split-from-nothing}), and (2) take a model on the original CID, and extend it to a model on the transformed CID by parameterizing the tree. For the second part, \autoref{def:model-construction} is almost the operation that we want. The only problem with it is that it sometimes assigns an extra boolean bit to the domain of the decision $D$. We need this extra bit in order to ensure that $D$ performs its task in case the root system 
\ryan{Not quite right, because referring to the root system makes it sound like  $X \to D$ is just in one place, and this only needs to be done once.  Maybe we should leave this line out in our next rewrite.}
\chris{but $X\to D$ IS in just one place, right? I'm not sure what the confusion is.}
\ryan{The confusion lies in the fact that you're parameterising multiple tasks.}
\chris{What multiple tasks? let's discuss, bc its not clear to me.}
has a non-directed info path. But for the purpose of usability, we would like the Taskify operation not to change the domain of any of the nodes in the original CID. This makes it easier to reason about the model using the Taskify lemma. We will fix this by doing one additional CID transformation, to make it so that this extra bit is in a different node, and porting the model to that transformed CID:~\looseness=-1




\begin{definition} [Transformation 4] \label{def:21jan30.2-fifth-transformation-to-split-root-decision}
Let $\sG^3=(\sV^3,E^3)$ be a CID \withSR with a tree  $T^3$.
Then $\splitfourth(\sG^3,T^3)=\sG^4$ 
where $\sG^4=(\sV^4,E^4)$
and the CID homomorphism $\hfourth\colon \sV^4 \to \sV^3$ are obtained from \autoref{le:21may19.2-CID-hom-from-node-copying-and-deleting}, by adding for each node $N$ a set of copies
    \[\sCopies(N) = \begin{cases} 
        \{(N,``\scopy")\} \casesif {$N=D^{\sRoot^{T^3}}$ and $\sRoot^{T^3}$ has non-directed info path}\\
        \emptyset \casesotherwise
    \end{cases}.\]
\end{definition}







\begin{definition} [Model adjustment for transformation 4] \label{def:21feb7.3-model-adjustment-after-fifth=transformation}
Let $\calM^3$ be the model from \autoref{def:model-construction} on a CID $\sG^3$ based on some $T^3$, $\calM^0$ and $\piTask^{D}$. Then we obtain a model $\calM^4$ on the CID $\sG^4=\splitfourth(\sG^3, T^3)$ as follows: If the root system has a directed info path, then $\sG^4 =\sG^3$ by definition and let $\calM^4=\calM^3$. If it has a non-directed info path, then $\calM^4$ is obtained from model $\calM^3$ by the following changes. 
\begin{itemize}
    \item Let $\dom^{\calM^4}((D,``\scopy"))=\bool$, and let $\dom^{\calM^4}(D)=\dom^{\calM^3}_\sbase(D)$.  

    \item Any chance node $N \in \Ch(D)$ is given $f^N_{\calM^4}(d,``\scopy",\pa^{\calM^4}(N)^-)=f^N_{\calM^3}((d,``\scopy"),\pa^{\calM^4}(N)^-)$, where $\pa^{\calM^4}(N)^-$ denotes the values of $\pa^{\calM^4}$ except for $d$ and $``\scopy"$, and $(d,``\scopy")$ denotes the concatenation of $d$ and $\scopy$.
    \chris{Is concatenation the right word here?}
\end{itemize}
\end{definition}




\begin{lemma} [$\calM^3$ and $\calM^4$ are equivalent] \label{le:21feb7.1-Transformation-4-produces-an-equivalent-model}
If model $\calM^4$ and homomorphism $\hfourth$ are obtained from a model $\calM^3$ on $\sG^3$ by \autoref{def:21jan30.2-fifth-transformation-to-split-root-decision}, then $\calM^3=\hfourth(\calM^4)$, i.e. it is the ported model of $\calM^4$ via $\hfourth$.
\end{lemma}


\begin{proof}
This follows directly by definition.
\end{proof}


Now we have all the ingredients needed to define the Taskify construction for a single decision. That is, the construction that assigns a task to a single decision.










\begin{definition} [Taskify Construction for a single decision] \label{def:taskify-construction-single}
The operation $\sTaskifySingle$ takes a CID $\sG$, a model $\sM$ on it, and for some decision $D$ a deterministic decision rule $\piTask^{D}$ that only depends on a single parent $X$ in the minimal d-reduction of $\sG$, and outputs a triple $\sTaskifySingle(\sG, M, \piTask^{D}) = (\GTaskify, \MTaskify, h)$ that are obtained as follows:
\begin{itemize}
    \item (Obtain a transformed CID with normal form tree) Let  $\sG^3=(\sV,\sE)$ be a CID
    with a normal form tree $T^3$ on it, and a homomorphism $\hfirsttolast$ from $\sG^3$ to $\sG$, where the root info-link $X^3 \to D^3$ of $T^3$ satisfies $h(X^3)=X$ and $h(D^3)=D$ (which exists by \autoref{le:20nov29.1-Existence-of-adequate-CID-split-from-nothing}). 
    
    \item (Parameterize this using the normal form tree) Let the model $\calM^3$ on $\sG^3$ be obtained by applying \autoref{def:model-construction} to the model $\sM$ on the nodes in $\sG$, using $\piTask^{D}$ and $T^3$.
    
    \item (Split the root decision) Define $\GTaskify=\splitfourth(\sG^3, T^3)$ with homomorphism $\hfourth$ from $\GTaskify$ to $\sG^3$ (from  \autoref{def:21jan30.2-fifth-transformation-to-split-root-decision}), and obtain $\MTaskify$ from $\calM^3$ according to \autoref{def:21feb7.3-model-adjustment-after-fifth=transformation}. Finally, let $h=\hfirsttolast\circ \hfourth$.
\end{itemize}
\end{definition}




\begin{definition} [Taskify Construction] \label{def:taskify-construction-full}
The operation $\sTaskify$ takes a CID $\sG$, a model $\sM$ on it, and for some set of decisions $\DTask\subseteq \sD$ 
a deterministic decision rule $\piTask^{D^i}$ for each $D^i \in \DTask$ that depends only on a single parent $X^i$ in the minimal
$d$-reduction of $\sG$, and outputs a triple $\sTaskify(\sG, M, \{\piTask^{D^i}\}) = (\GTaskify, \MTaskify, h)$ that are obtained as 
follows: Let $N=|\DTask|$ and let $D_1,...,D_N$ be the ordering of the decisions in $\DTask$ from latest to earliest according to the ordering of decision nodes in $\sG$.\footnote{Recall that there is such an ordering due to sufficient recall.} Then:
\begin{align*}
    (\GTaskify^0, \MTaskify^0,h^0) &= (\sG, \sM, \mathrm{id})\\
    (\GTaskify^{n+1}, \MTaskify^{n+1}, \tilde h^{n+1}) &= \sTaskifySingle(\GTaskify^n, \MTaskify^n, \piTask^{D_{n+1}})\\
    h^{n+1} &= \tilde h^{n+1}\circ h^n\\
    (\GTaskify, \MTaskify, h) &= (\GTaskify^N, \MTaskify^N, h^N)
\end{align*}
\end{definition}








Now we are able to prove the Taskify Lemma. In order to keep the lemma statement simple we first define the notion of a \textit{homomorphic extension} of a model. A homomorphic extension of a model on a graph $\sG$ is essentially a model on a super-graph of $\sG$ that agrees with the original w.r.t. the nodes in $\sG$. The taskify construction in fact produces a homomorphic extension of our original model as we will show, and transformation 4 was performed primarily to obtain that property.

\defHomomorphicExtension*

\begin{lemma}[Composition of Homomorphic extensions]\label{le:21-aug9.1-composition-of-homomorphic-extensions}Let $\sM^3$ on $\sG^3$ be a homomorphic extension of $\sM^2$ on $\sG^2$, and $\sM^2$ a homomorphic extension of $\sM^1$ on $\sG^1$. Then $\sM^3$ is a homomorphic extension of $\sM^1$. 
\end{lemma}

\begin{proof} Let $h^{2\gets 3}\colon \sG^3\to \sG^2$ and $h^{1\gets 2}\colon \sG^2\to \sG^1$ be the homomorphisms from the definition of homomorphic extension.
Firstly, since $\sG_1$ is a subgraph of $\sG_2$, and $\sG_2$ a subgraph of $\sG_3$. Hence clearly $\sG_1$ is a subgraph of $\sG_3$. Secondly, define $h^{1 \gets 3} = h^{1\gets 2} \circ h^{2\gets 3}$, which is also a homomorphism by the homomorphism composition lemma (\autoref{le:20dec7.1-composition-of-CID-splits}). Thirdly, since $\sM^1$ equals $\sM^2$ on the subgraph $\sG^1$, and $\sM^2$ equals $\sM^3$ on the subgraph $\sG^2$, and we know that $\sG^1$ is a subgraph of $\sG^2$, therefore $\sM^1$ equals $\sM^3$ on the subgraph $\sG^1$.
\end{proof}





\letaskify*

The proof will proceed as follows: We will show that the operation $\sTaskify$ produces a model $\MTaskify$ that satisfies the desired properties. Since $\sTaskify$ is built by iteratively 
assigning a task from the set of given tasks $\{\piTask^{D^i}\}$ using $\sTaskifySingle$ (in arbitrary order), we first (step 1) prove that $\sTaskifySingle$ produces a model that has the desired 
properties w.r.t. that single task. This result mostly follows from the properties we proved in the previous section (in particular that the decisions must perform their task, and that if they do, the utility nodes in the normal-form tree are constant with probability 1). However, it does not immediately follow from this 
that after iteratively applying $\sTaskifySingle$ $N$ times, all the decisions will perform their task, and that all utility nodes 
are constant: We have to show that a later application of $\sTaskifySingle$ does not adjust the model in a way so that the desired properties provided by an earlier application are no 
longer true. Therefore we must show (step 2), that after the $n+1^{\mathrm{th}}$ application of $\sTaskifySingle$, the decisions $D_1,...,D_n$ still have to perform their tasks 
$\piTask^{D_1},...,\piTask^{D_n}$, and that the utility nodes in the added normal-form trees for $X_1 \to D_1,...,X_n \to D_n$ are still constant with probability $1$. Intuitively, the reason this is true is that the $n+1^\text{th}$ application of $\sTaskifySingle$ only adds utility nodes that are constant, and doesn't change the model on existing nodes, which implies that the earlier added decisions face the same decision-problem, and hence still perform their task, and still cause the earlier-added utility nodes to be constant.


\begin{proof}
We will show that the operation $\sTaskify$ as defined in \autoref{def:taskify-construction-full} generates a triple $(\GTaskify, \MTaskify,h)=\sTaskify(\sG, \sM, \{\piTask^{D^i}\}_{D^i\in \DTask})$ that satisfies the desired properties, where $h$ is the required homomorphism for $\MTaskify$ to be a homomorphic extension of $\sM$.


We first (in step 1) show the result assuming that the decisions $\DTask$ to be provided with a task contains only a single decision $D$, so that $(\GTaskify, \MTaskify,h)= \sTaskifySingle(\sG, \sM, \piTask^{D})$. Since $\sTaskify$ is built up from repeated applications of $\sTaskifySingle$ we will use this in step 2 to show the general result by induction.



\textit{Step ($1$) : The result for a single task}. 
Assume that $\DTask$ contains only a single decision $D$, so that $(\GTaskify, \MTaskify,h)= \sTaskifySingle(\sG, \sM, \piTask^{D})$. 
Let $\Vadded= \VTaskify \setminus \sV$. We show each desired property in succession:

($\MTaskify$ is a homomorphic extension of $\sM$). Firstly, the graph $\sG$ is a subgraph of $\GTaskify$ directly by the definition of $\sTaskifySingle$ (\autoref{def:taskify-construction-single}). Secondly, by definition, $h=\hfirsttolast\circ \hfourth$, and since $\hfirsttolast$ and $\hfourth$ are homomorphic (\autoref{le:20nov29.1-Existence-of-adequate-CID-split-from-nothing}, \autoref{def:21jan30.2-fifth-transformation-to-split-root-decision}), so is $h$ (\autoref{le:20dec7.1-composition-of-CID-splits}). Thirdly, that $\MTaskify$ equals $\sM$ on the subgraph $\sG$ follows directly by definition of \autoref{def:model-construction} and \autoref{def:21jan30.2-fifth-transformation-to-split-root-decision} for all nodes except $D^i$, and if the root system of $T$ is directed then also for $D^i$. If it is non-directed, then the domain of $D^i$ has one boolean added to it in the model from \autoref{def:model-construction}, but we remove this in \autoref{def:21jan30.2-fifth-transformation-to-split-root-decision}.

\ref{le:21jan31.3a-taskify-optimal-iff-performs-task} {(\TaskifySublemmaPerformsTheirTaskName)} 
Firstly, by definition of $\sTaskifySingle$, $\MTaskify=\splitfourth(\sM^3)$, where $\sM^3$ is the standard
model obtained from a normal form tree as introduced in the beginning of \autoref{sec:model-definition}. 
We have already proven (\autoref{le:1.7-optimal-iff-truthful}) for $\sM^3$ that $D$ must perform its task under any optimal policy in the sense of \autoref{def:aug23.4-task-performance}. Hence, since $\calM^3=\hfourth(\MTaskify)$ (by \autoref{le:21feb7.1-Transformation-4-produces-an-equivalent-model}) so that $\MTaskify$ and $\sM^3$ are equivalent in the sense of \autoref{le:cidhom1-equivalence}, this implies that for any optimal policy on $\MTaskify$, that $\pi^{D^i}(a\mid\pa)=\piTask^{D^i}(x^i)$ as required.



\ref{le:21jan31.3c-taskify-added-utility-nodes-unaffected} {(\TaskifySublemmaAddedUtilityNodesName)}.
This is shown for $\calM^3$ in \autoref{le:1.7-optimal-iff-truthful}. Since $\calM^3=\hfourth(\MTaskify)$ (by \autoref{le:21feb7.1-Transformation-4-produces-an-equivalent-model}), so that for any policy $\spi$ on $\MTaskify$, the outcomes of $\MTaskify$ with $\spi$ and $\calM^3$ with ${\hfourth(\spi)}$ are equivalent in the sense of \autoref{le:cidhom1-equivalence}, therefore these models result in the same utility for any policy. Hence the same holds for $\MTaskify$.








\textit{Step ($2$) : The result for $N$ tasks}. 
Let $\Vadded^{n+1:n} = \VTaskify^{n+1} \setminus \VTaskify^n$ and  also $\Vadded^{n+1}=\VTaskify^{n+1} \setminus \sV$.
From step ($1$) it follows that for each $n$, the model $\MTaskify^{n}$ satisfies the desired properties relative to $\MTaskify^{n-1}$. That is, $\MTaskify^{n}$ is a homomorphic extension of $\MTaskify^{n-1}$ in which (a') $D_n$ must perform its task, and (b') the utility nodes in $\Vadded^{n:n-1}$ have a constant value. 
But we must show the stronger result that for each $n$, $\MTaskify^n$ is a homomorphic extension of $\sM$ in which (a) Each of $D_1, ...,D_n$ performs its task, and (b) the utility nodes in $\Vadded^n$ have a constant value. Intuitively, we must show that each application of $\sTaskifySingle$ doesn't undo the properties obtained by the previous applications.

We show these stronger properties by induction: We assume that they hold for $(\GTaskify^n, \MTaskify^n, h^n)$, and show that they hold for $(\GTaskify^{n+1}, \MTaskify^{n+1}, h^{n+1})$. Setting $n+1=N$ then finishes the proof.

($\MTaskify^{n+1}$ is a homomorphic extension of $\sM$). We know that $\MTaskify^{n+1}$ is a homomorphic extension of $\MTaskify^n$ from step (1), and that $\MTaskify^n$ is a homomorphic extension of $\sM$ from the induction assumption. Hence by \autoref{le:21-aug9.1-composition-of-homomorphic-extensions} $\MTaskify^{n+1}$ is a homomorphic extension of $\sM$. 

\ref{le:21jan31.3a-taskify-optimal-iff-performs-task} {(\TaskifySublemmaPerformsTheirTaskName)} Firstly, we know that for each utility node in in $\GTaskify^n$, its expected value in $\MTaskify^{n+1}$ equals that in $\MTaskify^n$, since by 
step ($1$) $\MTaskify^{n+1}$ is a homomorphic extension of $\MTaskify^{n}$. And for each added utility node in $\Vadded^{n+1}$, the value is constant, so long as the decision rules for $D_{n+1}$ and the decisions in $\Vadded^{n+1}$ are optimal again by step ($1$) \ref{le:21jan31.3c-taskify-added-utility-nodes-unaffected}. Hence the expected utility given each possible decision rule for $D_1,...,D_n$ is the same in $\MTaskify^{n+1}$ as in $\MTaskify^n$. Hence, since the induction assumption implies that for any optimal policy on $\MTaskify^n$, the decision rules for $D_1,...,D_n$ equal their tasks, the same holds for $\MTaskify^{n+1}$. 
Finally, that for any optimal policy on $\MTaskify^{n+1}$ the decision rule for $D_{n+1}$ is equal to its task follows directly by step ($1$) \ref{le:21jan31.3a-taskify-optimal-iff-performs-task}.



\ref{le:21jan31.3c-taskify-added-utility-nodes-unaffected} {(\TaskifySublemmaAddedUtilityNodesName)}
Take a policy $\pi$ for which each decision in $\{D_1,...,D_{n+1}\}\cup\Vadded^{n+1}$ has an optimal decision rule. Then in particular this holds for each decision in $\{D_{n+1}\}\cup \Vadded^{n+1:n}$, so that by step (1)(b), the 
utility nodes in $\Vadded^{n+1:n}$ have constant value in $\MTaskify^{n+1}$. Moreover, by step 1, $\MTaskify^{n+1}$ is a homomorphic extension of $\MTaskify^n$, so that in particular, $\GTaskify^{n}$ is a subgraph of $\GTaskify^{n+1}$ on which $\MTaskify^{n+1}$ equals $\MTaskify^n$, which implies that if we restrict $\pi$ to the subgraph $\GTaskify^n$ then this gives us a 
policy $\pi'$ for $\MTaskify^n$. Moreover, since $\pi$ had optimal decision rules for each decision in $\{D_1,...,D_{n+1}\}\cup\Vadded^{n+1}$ and hence also in $\{D_1,...,D_{n}\}\cup\Vadded^{n}$, and the utility of the nodes in $\Vadded^{n+1:n}$ are constant, this implies together with the equivalence between $\MTaskify^{n+1}$ and $\MTaskify^n$ that 
$\pi'$ is optimal on $\MTaskify^n$, which implies by the induction assumption that all utility nodes in $\Vadded^n$ are constant in $\MTaskify^n$. Since the model $\MTaskify^{n+1}$ is equal to $\MTaskify^n$ on the subset of nodes $\VTaskify^n$, this means that they are also constant in $\MTaskify^{n+1}$. 
\end{proof}




































    



==> theorems/Taskify-sublemmas.tex <==








\newcommand{\TaskifySublemmas}{
\begin{enumerate}[label=(\alph*)]
    \item \textbf{(Decisions are optimal iff they perform their task)} \label{le:21jan31.3a-taskify-optimal-iff-performs-task}
    If all decisions in $\Vadded$ have optimal decision rules with a policy $\pi$, then each $D^i$ is optimal under $\pi$ iff for all $\pa \in \dom(\Pa(D^i))$, if $P_\pi(\pa) > 0$, then $\pi^{D^i}(a | \pa) = t^i(x^i)$ with probability $1$, where $x^i$ is the value of $X^i$ assigned by $\pa$.
        
        
    \item \textbf{(Added utility nodes are unaffected by the original graph)} \label{le:21jan31.3c-taskify-added-utility-nodes-unaffected}
    Let $\{\pi^D\}_{D\in \sD'}$ 
    % \ryan{I know you didn't want to, but I still think it probably makes sense for it to say $D \in \sD'$, and then for us to specify what $\sD'$ is}
    %\chris{What about this?}
    % \ryan{it's better now imo}
    be a set of optimal decision rules for $\sD'=(\sD\cap \Vadded)\cup \{D^i\}_i^k$.
    % each decision $D$ in $\MTaskify$ that is also in $\Vadded$ or is one of $D^i$.
    Let $\{g^X\}_{X\in \sX'}$  for $\sX'\subseteq \sV$
    % \ryan{Likewise for $X \in \sX'$ here.}
    be any set of soft interventions where $X$ is a node in $\calG$, such that for all $D$, 
    $P(\Pa(D)_{g^X}=\pa^D)>1$ only if $P(\Pa(D)=\pa^D)>1$. Then $U_{g^X}=U = \max_\pa f^U_{\MTaskify}(\pa)$ with probability $1$ in ${\MTaskify}$.
    
    
    \item \textbf{(The model on the original nodes is unmodified)} \label{le:21jan31.3b-taskify-original-model-unchanged}
    For all nodes $V\in \sV$, 
    $\dom_{\MTaskify}(V)=\dom_M(V)$, and for all chance and utility nodes $V\in \sV$, $f^V_{\MTaskify}=f^V_M$.
   
    
    \item \textbf{(CID Homomorphism)} \label{le:21jan31.3d-taskify-homomorphic-split}
    There is a CID homomorphism $h$ from 
    $\GTaskify=(\VTaskify,\ETaskify)$ 
    to $\sG=(\sV,E)$ that has
    $h(V)\!=\!V$ for
    every node
    $V \in \sV \cap \VTaskify$ in both graphs.
\end{enumerate}
}

==> theorems/Taskify.tex <==






\begin{restatable}[Homomorphic extension]{definition}{defHomomorphicExtension}\label{le:21-may-19-Homomorphic-extension}
A CIM $\calM'$ on $\sG'$ is a \emph{homomorphic extension} of 
a CIM $\calM$ on $\sG$ if:
    i) $\sG$ is a subgraph of $\sG'$
    ii) there is a homomorphism $h\colon \sV'\ \to \sV$ 
    that has $h(V)=V$ for every node $V$ in $\sG$, and
    iii) $\calM'$ equals $\calM$ on the subgraph $\sG$.
\end{restatable}
\ryan{(iii) is not fully formal. Should we define (in a sentence) what it means for $\calM'$ to be restricted to $\calG$?}


\ryan{Maybe we should add a sentence here to introduce ``Taskify''?}


\newcommand{\TaskifySublemmaPerformsTheirTaskName}{Taskified decisions perform their task}
\newcommand{\TaskifySublemmaAddedUtilityNodesName}{Added utility nodes are constant}

\begin{restatable}[Taskify]{theorem}{letaskify}
\label{le:21jan31.3-multi-Taskify-lemma}
Let $\calM$ be a CIM on $\calG$, where $\DTask$ is a subset of the decision nodes. 
For each $D^i \in \DTask$, let $\piTask^{D^i}$ be a deterministic decision rule that depends only on a single parent $X^i$ in the minimal d-reduction of $\sG$. Then there is a homomorphic extension $\MTaskify$ of $\calM$, such that:~\looseness=-1
\begin{enumerate}[label=(\alph*)]
    \item \label{le:21jan31.3a-taskify-optimal-iff-performs-task} 
    (\TaskifySublemmaPerformsTheirTaskName)
    If a policy $\pi$ on $\MTaskify$ is optimal, then for all $D^i \in \DTask$, and all $\pa$ with $P_\pi(\pa) > 0$, the policy satisfies $\pi^{D^i}(a | \pa) = \piTask^{D^i} (a | x^i)$, where $x^i$ is the value of $X^i$ assigned by $\pa$.
    
    \item \label{le:21jan31.3c-taskify-added-utility-nodes-unaffected}
    (\TaskifySublemmaAddedUtilityNodesName)
    If a policy $\pi$ on $\MTaskify$ has optimal decision rules for all decisions in $\DTask \cup (\VTaskify \!\setminus \!\sV)$ then each utility node $U$ in $\VTaskify\setminus \sV$ has some $u \in \mathbb{R}$ such that $P^{\MTaskify}_{\pi}(U=u)=1$.
\end{enumerate}    
\ryan{Commented out the names of the Taskify conditions, to save two lines}




\end{restatable}


==> theorems/nonrequisite-removal.tex <==










\begin{restatable}[Optimal policy in the minimal $d$-reduction; {\citet{nilsson2000evaluating}}]{lemma}{lemmanonrequisiteremoval}%
\label{le:dred-performance}
Let 
$\calM$ be a model on 
$\calG$, a CID \withSR, 
that has $d$-reduction $\calG'$, 
Then, 
any optimal strategy for $\calM(\calG')$ is also optimal for $\calM$.
\end{restatable}





==> theorems/voc.tex <==










\begin{restatable}[VoC Criterion]{theorem}{theoremvoc}%
\label{thm:voc}
Let $\calG$ be a CID containing a chance node $X$.
There exists a CIM $\calM$ compatible with $\calG$ 
such that $X$ has 
strictly 
positive VoC %
if and only if the minimal d-reduction $\calG^*$,
contains a 
directed
path $X \pathto U$ for some $U \in \sU$.
\end{restatable}


